The Impacts of Mobility on Covid-19 Dynamics: Using Soft and Hard Data

This paper has the goal of evaluating how changes in mobility has affected the infection spread of Covid-19 throughout the 2020-2021 years. However, identifying a "clean" causal relation is not an easy task due to a high number of non-observable (behavioral) effects. We suggest the usage of Google Trends and News-based indexes as controls for some of these behavioral effects and we find that a 1\% increase in residential mobility (i.e. a reduction in overall mobility) have significant impacts for reducing both Covid-19 cases (at least 3.02\% on a one-month horizon) and deaths (at least 2.43\% at the two-weeks horizon) over the 2020-2021 sample. We also evaluate the effects of mobility on Covid-19 spread on the restricted sample (only 2020) where vaccines were not available. The results of diminishing mobility over cases and deaths on the restricted sample are still observable (with similar magnitudes in terms of residential mobility) and cumulative higher, as the effects of restricting workplace mobility turns to be also significant: a 1\% decrease in workplace mobility diminishes cases around 1\% and deaths around 2\%.

==> Resultados/resultado_mun_dinpan_not.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{7}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}\\
            &\multicolumn{1}{c}{cases}&\multicolumn{1}{c}{cases}&\multicolumn{1}{c}{cases}&\multicolumn{1}{c}{cases}&\multicolumn{1}{c}{deaths}&\multicolumn{1}{c}{deaths}&\multicolumn{1}{c}{deaths}\\
            &         m=1         &         m=2         &         m=3         &         m=4         &         m=2         &         m=3         &         m=4         \\
\hline
cases\_1  &      -0.404\sym{***}&      -0.426\sym{***}&      -0.446\sym{***}&      -0.467\sym{***}&                     &                     &                     \\
            &    (0.0131)         &    (0.0136)         &    (0.0145)         &    (0.0156)         &                     &                     &                     \\
[1em]
cases\_2 &      -0.125\sym{***}&      -0.147\sym{***}&      -0.180\sym{***}&      -0.205\sym{***}&                     &                     &                     \\
            &    (0.0130)         &    (0.0136)         &    (0.0148)         &    (0.0160)         &                     &                     &                     \\
[1em]
cases\_3 &     -0.0223         &     -0.0394\sym{**} &     -0.0698\sym{***}&     -0.0920\sym{***}&                     &                     &                     \\
            &    (0.0119)         &    (0.0123)         &    (0.0132)         &    (0.0140)         &                     &                     &                     \\
[1em]
cases\_4 &      0.0150         &     0.00667         &     -0.0133         &     -0.0241\sym{*}  &                     &                     &                     \\
            &    (0.0101)         &    (0.0102)         &    (0.0110)         &    (0.0115)         &                     &                     &                     \\
[1em]
residential &     -0.0383\sym{***}&     -0.0175\sym{***}&     -0.0195\sym{***}&     0.00442         &     -0.0411\sym{***}&     -0.0643\sym{***}&     -0.0619\sym{***}\\
            &   (0.00472)         &   (0.00457)         &   (0.00513)         &   (0.00475)         &   (0.00677)         &   (0.00841)         &   (0.00787)         \\
[1em]
workplace   &    0.000742         &     0.00233\sym{*}  &    -0.00359\sym{**} &   -0.000692         &    -0.00308         &    -0.00500\sym{*}  &    -0.00414         \\
            &   (0.00123)         &   (0.00118)         &   (0.00135)         &   (0.00130)         &   (0.00179)         &   (0.00224)         &   (0.00215)         \\
[1em]
1st\_dose    &    -0.00271         &     -0.0195\sym{***}&    -0.00432         &      0.0113\sym{*}  &     -0.0258\sym{***}&     -0.0277\sym{***}&     -0.0103         \\
            &   (0.00541)         &   (0.00565)         &   (0.00549)         &   (0.00516)         &   (0.00768)         &   (0.00765)         &   (0.00730)         \\
[1em]
2nd\_dose    &      0.0180\sym{***}&      0.0120\sym{***}&      0.0230\sym{***}&      0.0124\sym{***}&    -0.00184         &     0.00845\sym{*}  &      0.0175\sym{***}\\
            &   (0.00315)         &   (0.00301)         &   (0.00300)         &   (0.00334)         &   (0.00415)         &   (0.00424)         &   (0.00431)         \\
[1em]
n\_covid     &    -0.00122\sym{***}&   -0.000646\sym{**} &    -0.00105\sym{***}&    0.000751\sym{**} &    -0.00127\sym{***}&    -0.00167\sym{***}&    -0.00206\sym{***}\\
            &  (0.000227)         &  (0.000231)         &  (0.000244)         &  (0.000230)         &  (0.000339)         &  (0.000358)         &  (0.000330)         \\
[1em]
n\_prevention&   -0.000369         &     0.00177\sym{*}  &     0.00210\sym{*}  &    -0.00119         &   -0.000777         &     0.00107         &     0.00351\sym{**} \\
            &  (0.000786)         &  (0.000798)         &  (0.000826)         &  (0.000787)         &   (0.00115)         &   (0.00128)         &   (0.00116)         \\
[1em]
n\_fakenews  &    -0.00936         &    -0.00310         &    -0.00702         &     0.00839         &     -0.0170\sym{*}  &    -0.00569         &     -0.0151\sym{*}  \\
            &   (0.00516)         &   (0.00503)         &   (0.00484)         &   (0.00493)         &   (0.00661)         &   (0.00697)         &   (0.00696)         \\
[1em]
n\_vaccines  &    0.000242         &  -0.0000326         &   -0.000359         &   -0.000728\sym{*}  &     0.00156\sym{**} &     0.00107\sym{*}  &    0.000587         \\
            &  (0.000346)         &  (0.000362)         &  (0.000351)         &  (0.000353)         &  (0.000504)         &  (0.000522)         &  (0.000493)         \\
[1em]
gt\_covid    &    0.000168\sym{***}&   -0.000262\sym{***}&   -0.000259\sym{***}&   -0.000514\sym{***}&    0.000526\sym{***}&    0.000269\sym{***}&    0.000118         \\
            & (0.0000504)         & (0.0000474)         & (0.0000478)         & (0.0000483)         & (0.0000672)         & (0.0000649)         & (0.0000622)         \\
[1em]
gt\_prevention&    0.000107         &    0.000441\sym{***}&   -0.000434\sym{***}&   -0.000276\sym{**} &    0.000582\sym{***}&    0.000370\sym{**} & -0.00000737         \\
            &  (0.000107)         &  (0.000101)         &  (0.000102)         & (0.0000999)         &  (0.000145)         &  (0.000133)         &  (0.000135)         \\
[1em]
gt\_fakenews &   -0.000738\sym{***}&   -0.000474\sym{***}&   -0.000192         &   0.0000251         &  -0.0000371         &  -0.0000987         &   -0.000390\sym{*}  \\
            &  (0.000127)         &  (0.000120)         &  (0.000117)         &  (0.000126)         &  (0.000157)         &  (0.000166)         &  (0.000157)         \\
[1em]
gt\_vaccines &   -0.000143         &    0.000148         &    0.000206\sym{*}  &    0.000657\sym{***}&   -0.000758\sym{***}&   -0.000591\sym{***}&   -0.000573\sym{***}\\
            & (0.0000855)         & (0.0000813)         & (0.0000890)         & (0.0000880)         &  (0.000117)         &  (0.000123)         &  (0.000123)         \\
[1em]
trend       &     -0.0264\sym{***}&     -0.0265\sym{***}&     -0.0300\sym{***}&     -0.0385\sym{***}&    -0.00740\sym{**} &    -0.00963\sym{**} &     -0.0156\sym{***}\\
            &   (0.00185)         &   (0.00208)         &   (0.00218)         &   (0.00243)         &   (0.00264)         &   (0.00316)         &   (0.00308)         \\
[1em]
deaths\_1 &                     &                     &                     &                     &      -0.523\sym{***}&      -0.523\sym{***}&      -0.538\sym{***}\\
            &                     &                     &                     &                     &    (0.0132)         &    (0.0131)         &    (0.0135)         \\
[1em]
deaths\_2&                     &                     &                     &                     &      -0.227\sym{***}&      -0.221\sym{***}&      -0.240\sym{***}\\
            &                     &                     &                     &                     &    (0.0154)         &    (0.0150)         &    (0.0153)         \\
[1em]
deaths\_3&                     &                     &                     &                     &     -0.0822\sym{***}&     -0.0719\sym{***}&     -0.0837\sym{***}\\
            &                     &                     &                     &                     &    (0.0144)         &    (0.0141)         &    (0.0143)         \\
[1em]
deaths\_4&                     &                     &                     &                     &     -0.0379\sym{***}&     -0.0269\sym{*}  &     -0.0241\sym{*}  \\
            &                     &                     &                     &                     &    (0.0111)         &    (0.0112)         &    (0.0112)         \\
[1em]
\_cons      &       1.599\sym{***}&       1.880\sym{***}&       2.110\sym{***}&       2.219\sym{***}&       0.476\sym{***}&       1.109\sym{***}&       1.620\sym{***}\\
            &    (0.0831)         &    (0.0955)         &     (0.104)         &     (0.117)         &     (0.116)         &     (0.129)         &     (0.133)         \\
\hline
N           &       15966         &       15363         &       14752         &       14130         &       11288         &       10922         &       10543         \\
p           &           0         &           0         &           0         &   4.94e-324         &           0         &           0         &           0         \\
\hline\hline
\multicolumn{8}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{8}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}


==> Resultados/resultado_mun_dinpan_srag.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{7}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}\\
            &\multicolumn{1}{c}{cases}&\multicolumn{1}{c}{cases}&\multicolumn{1}{c}{cases}&\multicolumn{1}{c}{cases}&\multicolumn{1}{c}{deaths}&\multicolumn{1}{c}{deaths}&\multicolumn{1}{c}{deaths}\\
            &         m=1         &         m=2         &         m=3         &         m=4         &         m=2         &         m=3         &         m=4         \\
\hline
cases\_1  &      -0.347\sym{***}&      -0.475\sym{***}&      -0.466\sym{***}&      -0.497\sym{***}&                     &                     &                     \\
            &    (0.0177)         &    (0.0182)         &    (0.0191)         &    (0.0186)         &                     &                     &                     \\
[1em]
cases\_2 &      -0.120\sym{***}&      -0.202\sym{***}&      -0.220\sym{***}&      -0.258\sym{***}&                     &                     &                     \\
            &    (0.0189)         &    (0.0205)         &    (0.0224)         &    (0.0210)         &                     &                     &                     \\
[1em]
cases\_3 &     -0.0133         &     -0.0693\sym{***}&     -0.0657\sym{**} &      -0.121\sym{***}&                     &                     &                     \\
            &    (0.0172)         &    (0.0193)         &    (0.0215)         &    (0.0221)         &                     &                     &                     \\
[1em]
cases\_4 &     0.00770         &    -0.00646         &     0.00563         &     -0.0260         &                     &                     &                     \\
            &    (0.0121)         &    (0.0141)         &    (0.0154)         &    (0.0163)         &                     &                     &                     \\
[1em]
residential &     -0.0347\sym{***}&     -0.0363\sym{***}&     -0.0135         &    -0.00460         &     -0.0377\sym{***}&     -0.0699\sym{***}&     -0.0717\sym{***}\\
            &   (0.00553)         &   (0.00675)         &   (0.00693)         &   (0.00607)         &   (0.00937)         &    (0.0103)         &    (0.0154)         \\
[1em]
workplace   &   -0.000667         &   -0.000557         &   -0.000490         &  -0.0000686         &   -0.000203         &    -0.00448         &    -0.00964\sym{*}  \\
            &   (0.00144)         &   (0.00170)         &   (0.00179)         &   (0.00163)         &   (0.00243)         &   (0.00283)         &   (0.00400)         \\
[1em]
srag\_vac    &      -0.181\sym{***}&     -0.0175         &     -0.0205         &    -0.00879         &      0.0348\sym{*}  &     0.00542         &     -0.0272         \\
            &    (0.0106)         &    (0.0108)         &    (0.0116)         &    (0.0116)         &    (0.0140)         &    (0.0143)         &    (0.0152)         \\
[1em]
n\_covid     &    -0.00119\sym{***}&    -0.00147\sym{***}&    -0.00123\sym{***}&    0.000262         &   -0.000560         &    -0.00163\sym{***}&    -0.00217\sym{***}\\
            &  (0.000303)         &  (0.000293)         &  (0.000323)         &  (0.000306)         &  (0.000408)         &  (0.000420)         &  (0.000398)         \\
[1em]
n\_prevention&    -0.00181\sym{*}  &    0.000649         &     0.00135         &    -0.00200\sym{*}  &    -0.00165         &     0.00101         &     0.00151         \\
            &  (0.000879)         &  (0.000900)         &  (0.000970)         &  (0.000890)         &   (0.00136)         &   (0.00138)         &   (0.00134)         \\
[1em]
n\_fakenews  &     -0.0109\sym{*}  &      0.0109\sym{*}  &    -0.00874         &     0.00538         &     -0.0147\sym{*}  &    -0.00931         &     -0.0136         \\
            &   (0.00459)         &   (0.00514)         &   (0.00502)         &   (0.00497)         &   (0.00705)         &   (0.00711)         &   (0.00741)         \\
[1em]
n\_vaccines  &   -0.000319         &    0.000698         &     0.00128\sym{**} &   -0.000957\sym{*}  &    0.000184         &     0.00112         &     0.00136\sym{*}  \\
            &  (0.000423)         &  (0.000411)         &  (0.000428)         &  (0.000442)         &  (0.000564)         &  (0.000591)         &  (0.000607)         \\
[1em]
gt\_covid    &    0.000196\sym{***}&   -0.000288\sym{***}&   -0.000294\sym{***}&   -0.000633\sym{***}&    0.000459\sym{***}&    0.000336\sym{***}&    0.000230\sym{**} \\
            & (0.0000580)         & (0.0000597)         & (0.0000629)         & (0.0000612)         & (0.0000844)         & (0.0000829)         & (0.0000863)         \\
[1em]
gt\_prevention&  -0.0000878         &    0.000122         &   -0.000291\sym{*}  &   0.0000505         &    0.000858\sym{***}&    0.000378\sym{*}  &   0.0000160         \\
            &  (0.000131)         &  (0.000141)         &  (0.000141)         &  (0.000137)         &  (0.000194)         &  (0.000193)         &  (0.000193)         \\
[1em]
gt\_fakenews &   -0.000719\sym{***}&   0.0000268         &   -0.000144         &    0.000120         &    0.000151         &  -0.0000939         &   -0.000489\sym{*}  \\
            &  (0.000134)         &  (0.000138)         &  (0.000152)         &  (0.000151)         &  (0.000196)         &  (0.000196)         &  (0.000192)         \\
[1em]
gt\_vaccines &   -0.000196\sym{*}  &   0.0000999         &    0.000170         &    0.000807\sym{***}&   -0.000863\sym{***}&   -0.000511\sym{***}&   -0.000863\sym{***}\\
            & (0.0000958)         &  (0.000104)         &  (0.000107)         &  (0.000104)         &  (0.000129)         &  (0.000146)         &  (0.000145)         \\
[1em]
trend       &     -0.0557\sym{***}&     -0.0363\sym{***}&     -0.0357\sym{***}&     -0.0419\sym{***}&     -0.0168\sym{***}&     -0.0266\sym{***}&     -0.0214\sym{***}\\
            &   (0.00389)         &   (0.00372)         &   (0.00393)         &   (0.00429)         &   (0.00402)         &   (0.00503)         &   (0.00529)         \\
[1em]
deaths\_1 &                     &                     &                     &                     &      -0.570\sym{***}&      -0.570\sym{***}&      -0.594\sym{***}\\
            &                     &                     &                     &                     &    (0.0163)         &    (0.0167)         &    (0.0187)         \\
[1em]
deaths\_2&                     &                     &                     &                     &      -0.260\sym{***}&      -0.267\sym{***}&      -0.300\sym{***}\\
            &                     &                     &                     &                     &    (0.0195)         &    (0.0197)         &    (0.0220)         \\
[1em]
deaths\_3&                     &                     &                     &                     &     -0.0857\sym{***}&     -0.0831\sym{***}&      -0.117\sym{***}\\
            &                     &                     &                     &                     &    (0.0188)         &    (0.0191)         &    (0.0201)         \\
[1em]
deaths\_4&                     &                     &                     &                     &     -0.0175         &    -0.00616         &     -0.0259         \\
            &                     &                     &                     &                     &    (0.0143)         &    (0.0153)         &    (0.0154)         \\
[1em]
\_cons      &       3.532\sym{***}&       2.648\sym{***}&       2.472\sym{***}&       2.739\sym{***}&       0.805\sym{***}&       1.826\sym{***}&       2.087\sym{***}\\
            &     (0.209)         &     (0.200)         &     (0.215)         &     (0.231)         &     (0.209)         &     (0.249)         &     (0.251)         \\
\hline
N           &        9940         &        9393         &        8810         &        8200         &        7615         &        7232         &        6802         \\
p           &   5.44e-291         &   9.64e-203         &   1.46e-194         &   1.67e-217         &           0         &   6.09e-319         &   8.58e-282         \\
\hline\hline
\multicolumn{8}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{8}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}

